IBIA: An Incremental Build-Infer-Approximate Framework for Approximate Inference of Partition Function

Exact computation of the partition function is known to be intractable, necessitating approximate inference techniques. Existing methods for approximate inference are slow to converge for many benchmarks. The control of accuracy-complexity trade-off is also non-trivial in many of these methods. We propose a novel incremental build-infer-approximate (IBIA) framework for approximate inference that addresses these issues. In this framework, the probabilistic graphical model is converted into a sequence of clique tree forests (SCTF) with bounded clique sizes. We show that the SCTF can be used to efficiently compute the partition function. We propose two new algorithms which are used to construct the SCTF and prove the correctness of both. The first is an algorithm for incremental construction of CTFs that is guaranteed to give a valid CTF with bounded clique sizes and the second is an approximation algorithm that takes a calibrated CTF as input and yields a valid and calibrated CTF with reduced clique sizes as the output. We have evaluated our method using several benchmark sets from recent UAI competitions and our results show good accuracies with competitive runtimes.

==> reply2.tex <==


\begin{itemize}
    \item \textbf{Intuition of where the ideas presented come from}: Looking at the paper again, we feel that our section on related work is a little fragmented and the motivation of our approach is lost. To make it clear, we can add a subsection in Section 3 that describes the motivation of the approach before giving the overview.
    %, and also add a more detailed comparison with related work. 
    %Section on related work is a little fragmented. We can add motivation. 

    \item \textbf{Why will it work better than existing approaches:} None of the existing approaches that use multiple CTs can be used for the estimation of the partition function. Most of the existing variational methods for PR estimation perform iterative BP on loopy cluster graphs that are constructed based on the graph structure of the PGMs. In contrast, approximations in IBIA are based on both factor-based and structure-based information which results in better accuracies. Moreover, since IBIA uses clique trees instead of cluster graphs the belief propagation step is non-iterative, which makes it fast. We can emphasize this in the introduction. 

    \item Impact of paramet
\end{itemize}

The inference approaches presented in Xiang et al. (1993), Xiang \& Lesser (2003) and Murphy (2002) divide the graph structure corresponding to the PGM but do not guarantee bounded clique sizes. Bhanja \& Ranganthan (2004) present an iterative method to divide the network structure. Starting with a subgraph over a fixed number of variables, the network size is iteratively modified by adding or removing variables until the maximum clique size in the corresponding CTF is less than the user-specified bound. However, in each iteration, the entire subgraph needs to be re-triangulated to find the corresponding CTF, which is compute-intensive. 
In contrast, IBIA uses an incremental build strategy for dividing the PGM. It starts with an initial CTF that contains a disjoint subset of factors and incrementally modifies smaller portions of the CT to add new factors until the clique sizes remain bounded. This reduces the effort required for re-triangulation.


The method proposed in Murphy (2002) uses CTFs corresponding to each time slice in the 2T-BN representation of a dynamic BN. Beliefs are transferred from one CT to the next using joint beliefs over clusters of variables present in both CTFs (Boyen \& Koller, 1998). However, this approximation does not guarantee that the generated clusters form a connected CT and hence, need not preserve the partition function. Therefore, this approximation technique cannot be used to estimate partition function.
In Bhanja \& Ranganthan (2004), the information is transmitted from one CTF to the next using an approximate Chow-Liu tree, containing variables present in both CTFs.  However, this method is applicable only when beliefs are normalized. Extension to handle un-normalized beliefs is not straightforward. Moreover, in this method, the creation of the Chow-Liu tree  requires the computation of mutual information (MI) between pairs of interface variables that are in close proximity in the graph structure of the PGM. However, these variables could be present in different cliques in the corresponding CT. Therefore, the computation of MI could become expensive in terms of both time and memory.
In contrast, in IBIA, the beliefs are transferred via the approximate CTF which is constructed based on metrics that require computation of MI only between variables that are present within the same clique. This reduces the  complexity of the approach. 
The approximate CTF in IBIA contains both interface and non-interface variables, and the clique sizes are bounded by a user-defined value, $mcs_{im}$ instead of a fixed value of 2 in the case of Chow-Liu trees. This allows for a better approximation of the joint distribution of the interface variables which in turn results in improved accuracy. 

==> tikz/libdai.tex <==
\begin{figure}[!htbp]
 \centering
     \begin{tikzpicture}
        \begin{axis}[ylabel={Error}, xlabel={\#Instances (out of 97)}, ymax=20,legend pos=outer north east,legend cell align=left,legend style={font=\scriptsize}]
        \addplot[blue,line width=1.5pt] table [x=P, y=LBP, col sep=comma] {libdai/libdai.csv}; 
        %\addlegendentry{Loopy Belief Propagation}
        \addlegendentry{LBP}
        \addplot[cyan,line width=1.5pt] table [x=P, y=TREEEP, col sep=comma] {libdai/libdai.csv}; 
        \addlegendentry{Tree Expectation Propagation}
        %\addlegendentry{TREEEP}
        \addplot[orange,line width=1.5pt] table [x=P, y=GBP_MIN, col sep=comma] {libdai/libdai.csv}; 
        %\addlegendentry{Genaralized Belief Propagation (GBP) with minimum clusters}
        \addlegendentry{GBP with minimum sized clusters}
        %\addlegendentry{GBP\_MIN}
        \addplot[magenta,line width=1.5pt] table [x=P, y=HAK_MIN, col sep=comma] {libdai/libdai.csv}; 
        \addlegendentry{Double-loop GBP with minimum sized clusters}
        %\addlegendentry{HAK\_MIN}
        \addplot[pink,line width=1.5pt] table [x=P, y=HAK_LOOP3, col sep=comma] {libdai/libdai.csv}; 
        \addlegendentry{Double-loop GBP with $loopdepth=3$}
        %\addlegendentry{HAK\_LOOP3}
        \addplot[teal,line width=1.5pt] table [x=P, y=WMB20, col sep=comma] {libdai/libdai.csv}; 
        %\addlegendentry{Weighted Mini Bucket elimination with $ibound=20$}
        %\addlegendentry{WMB}
        \addlegendentry{WMB with $ibound=20$}
        \addplot[red,line width=1.5pt] table [x=P, y=IBIA20, col sep=comma] {libdai/libdai.csv}; 
        \addlegendentry{IBIA with $mcs_p=20$}
        \addplot[black,line width=1.5pt] table [x=P, y=IJGPSS, col sep=comma] {libdai/libdai.csv}; 
        %\addlegendentry{Sample search with $ibound=20$ and $w\mbox{-}cutset~bound=20$ }
        \addlegendentry{IJGPSS with $ibound=20$ and $w\mbox{-}cutset~bound=20$ }
        %\addlegendentry{IJGPSS}
        \end{axis}
     \end{tikzpicture}
    \caption{Cactus plot for error in $\log_{10}(PR)$ obtained using different inference techniques for BN benchmarks with runtime limit set to 20 minutes. \textcolor{red}{Remove IBIA?}}
    \label{fig:bn.libdai}
\end{figure}

